An Optimization-Based Inverse Kinematics Solver for Continuum Manipulators in Intricate Environments

Continuum manipulators have gained significant attention as a promising alternative to rigid manipulators, offering notable advantages in terms of flexibility and adaptability within intricate workspace. However, the broader application of high degree-of-freedom (DoF) continuum manipulators in intricate environments with multiple obstacles necessitates the development of an efficient inverse kinematics (IK) solver specifically tailored for such scenarios. Existing IK methods face challenges in terms of computational cost and solution guarantees for high DoF continuum manipulators, particularly within intricate workspace that obstacle avoidance is needed. To address these challenges, we have developed a novel IK solver for continuum manipulators that incorporates obstacle avoidance and other constraints like length, orientation, etc., in intricate environments, drawing inspiration from optimization-based path planning methods. Through simulations, our proposed method showcases superior flexibility, efficiency with increasing DoF, and robust performance within highly unstructured workspace, achieved with acceptable latency.

==> sections/conclusion.tex <==
Our approach addresses the challenges posed by continuum manipulators' highly redundant structure by treating them as systems of continuous paths. Central to our methodology is the development of an IK solver capable of addressing various demands, such as end orientation tracking, length control, and intricate obstacle avoidance. The algorithm achieves an $O(n^2)$ complexity, making it practical for manipulators with varying numbers of segments and high degrees of freedom.
Experimental results demonstrate the efficiency and effectiveness of our approach, showing competitive time consumption and the ability to reach local optimization quickly during path tracking in intricate environments. Moreover, we demonstrate the solver's effectiveness in enabling continuum manipulators to track paths in challenging real-world scenarios, thereby enhancing manipulator performance and safety.

Future research directions include further optimization of the IK solver to improve efficiency and convergence speed, especially in scenarios with significant initial guess deviations. Additionally, we plan to explore advanced optimization methods, such as conjugate gradient descent, adaptive optimization, or accelerated gradient descent, to enhance the efficiency of our optimization process.
Furthermore, we aim to extend our approach to consider dynamic obstacles and enable real-time re-planning for more robust and adaptive continuum manipulator planning and control. Ultimately, we plan to develop a novel motion planning method for continuum robot arms based on our IK solver, enabling them to navigate intricate environments in real-time.

==> sections/old-sections/experiments.tex <==
% \subsection{success rate of constant length inverse kinematics/ or the length convergence result}
% \ys{yeah just constant length, show that we can do it, and the succuess rate might not be great}

% different length

% or maybe just delete this part

\subsection{Time Consumption Regarding Number of Segments}
% \ys{we run the stuff for continuum manipulators with different number of segments, different number of path points, and compare the time consumption}

% In this section, we would like to talk about the time consumption of each part of the algorithm, with regard to different settings of the parameters, the number of segments and the number of path points.
% We tried the experiment on several different settings of obstacles (some examples shown in Figure~\ref{obs}). The we repeat experiment under each setting for 10 times, and we calculate the mean value of time consumption.
% As a result, the time consumption of path planning part, arc fitting part, and the total, and the ratio, with relate to different number of segments are listed below in Table~\ref{table:time_consumption}, $N$ represents the number of segments, $t_p$ represents the time consumption of path generation, $t_c$ represents the time consumption of length control, $T$ represents the total time consumption, $r_p$ represents the ratio between $t_p$ and $T$, $r_c$ represents the ratio between $t_c$ and $T$. During the experiment, the total length of the continuum manipulator is set to be the same. All the experiments are conducted in MATLAB.

In this section, we delve into an evaluation of the computational efficiency of our algorithm by examining the time consumption across various parameter settings, including segment numbers and path points. Our experiments encompass a range of obstacle configurations (examples shown in Figure~\ref{obs}). For each configuration, we conducted ten repetitions of the experiment and computed the mean time consumption.

The results are summarized in Table~\ref{table:time_consumption}, where $N$ represents the number of segments, $t_p$ denotes the time consumption during path generation, $t_c$ corresponds to the time consumed by the arc length control step, and $T$ reflects the total time consumption. Additionally, we present $r_p$, the ratio of $t_p$ to $T$, and $r_c$, the ratio of $t_c$ to $T$. It's worth noting that throughout the experiments, the total length of the continuum manipulator remained constant. All experiments were conducted in MATLAB.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{Figure/obs.png}
    \caption{Experiments in different settings of obstacles. The blue curve represents the path generated in the prior step, while the yellow piecewise arc spline with $G^1$ continuity represents the configuration of the continuum manipulator.
}      
    \label{obs}
\end{figure}

\begin{table}
    \caption{Time consumption} % title of Table
	\centering % used for centering table
	\begin{tabular}{l l l l l l} % centered columns (4 columns)
		\hline\hline %inserts double horizontal lines
		 $N$ & $t_p [s]$ & $t_c [s]$ & $T [s]$ & $r_p$ & $r_c$\\ [1.0ex]
		\hline % inserts single horizontal line
  
     5& 0.3042 & 0.0173 & 0.3215 & 94.62\% & 5.38\%\\[1.0ex]
     6& 0.3063 & 0.0212 & 0.3275 & 93.53\% & 6.47\%\\[1.0ex]
     7& 0.3041 & 0.0289 & 0.3330 & 91.32\% & 8.68\%\\[1.0ex]
     8& 0.3039 & 0.0335 & 0.3374 & 90.07\% & 9.93\%\\[1.0ex]
     9& 0.3025 & 0.0392 & 0.3417 & 88.52\% & 11.48\%\\[1.0ex]
     10& 0.3029 & 0.0468 & 0.3479 & 86.62\% & 13.38\%\\[1.0ex]
    
    \hline %inserts single line
	\end{tabular}
	\label{table:time_consumption} % is used to refer this
\end{table}

% Considering the data, we have the discussion below: the path plan process take the major part of the time consumption, and that the time consumption doesn't increase too much when number of segment increase.

% Now let's talk about how to make the time consumption shorter. Since path generation take the major part, the time consumption can reduce time consumption by use less path points, or reduce the iteration number make it stop once the path is good enough. Or make the CHOMP path planning more efficient, since I right it my self, and this part take like around 90 percent of the time cost, so there's a great potential in this method. Also, CHOMP is utilized since it can be optimized considering the length, curvature, etc, but sampling based method like RRT might also work in this frame, and maybe we can make it more efficient.
Analyzing the data, we observe that the path planning phase constitutes the major portion of time consumption. Remarkably, as the number of segments increases, the time consumption does not exhibit a significant increment.

To improve computational efficiency, we propose several avenues. Given that path generation dominates the time consumption, one strategy is to reduce the number of path points or implement stopping criteria that halt the process when an adequately optimal path is identified. Furthermore, optimizing the CHOMP path planning component holds significant potential, as it currently accounts for approximately 90 percent of the time cost. Exploring alternatives such as sampling-based methods like Rapidly-exploring Random Trees (RRT) within this framework may also offer enhanced efficiency prospects.

\subsection{End Effector Path Tracking}
% run the robot end effector to track a circle, that the continuum manipulator go through an unstructured environment.
% Use obs5 for 5-10 segments maybe? and use obs3 (go through the center maybe)


% In this section, we set the continuum manipulator in an unstructured environment. The total length of the continuum manipulator is set to be the same, while the number of segments are set from 5 to 10. During the experiment, we generate the trajectory for the end-effector, and take the same initial setting for 'active obstacle' process for each IK solving process, then just calculate the continuum manipulator configuration with our IK solver, for the waypoint on the end effector, one by one.


% As a result, we demonstrate that our IK sovler can help to track the end effector path, while the main body are through a complex and unstructured environments. We also tried different number of segment to track, and the latency is around 0.3~s.
% The tracking process of 5 segments setting and 10 segments setting are shown in Figure~\ref{track}. The rest settings from 6 segments to 9 segments are included in the supplementary video.
In this experiment, we set the continuum manipulator within an intricate environment with multiple obstacles, while maintaining a consistent total length for the manipulator. We vary the number of segments, ranging from 5 to 10, to assess performance under diverse conditions. Throughout the experiments, we initialize the 'active obstacle' process consistently for each IK solving process. Subsequently, we calculate the continuum manipulator's configuration to match the end-effector waypoints sequentially.

The outcomes of this experiment unequivocally demonstrate the effectiveness of our IK solver in accurately tracking the end-effector path, even in complex and unstructured environments. We extended our investigation to different segment configurations, and consistently observed latencies of approximately 0.3 seconds during the tracking process.

Figure~\ref{track} showcases the end-effector tracking processes for settings involving 5 and 10 segments. Experiments with segment counts ranging from 6 to 9, is available in the supplementary video.
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{Figure/track.png}
    \caption{The blue curve represents the path generated in the prior step, while the yellow piecewise arc spline with $G^1$ continuity represents the configuration of the continuum manipulator. A) Continuum manipulator with 5 segments. B) Continuum manipulator with 10 segments.
}      
    \label{track}
\end{figure}

==> sections/old-sections/old-circuit_signal-flow.tex <==
% shrink this section. Only keep the latest circuit version

% Each origami continuum module consists of a compliant plastic body, an acrylic end plate, and a custom-made PCB, using an 8-bit ATmega32U4 as microprocessor, for embedded control. Further, a total of four electrical wires run through the cavity of the origami structure in a helical shape, providing power and communication between continuum modules. The module control boards communicate to a desktop computer by using Inter-Integrated Circuit (I2C) protocol. 

% When a motor retracts its cable, while the other two keep still, the differences in cable length will clearly cause the origami module to bend towards the shorter cable. Identically, if all three motors retract their cables, the entire module will contract axially. The motors and cables are mounted in a triangular pattern, giving each module a full 3 degrees of freedom (DoF) in the form of bending curvature, bending direction, and segment length. More detail the kinematics of the module can be found in our prior work \cite{santoso2017design}. The controller board contains three channels of motor drivers, each of which being able to receive encoder data from the motor and implement low-level feedback control on the cable lengths.  

The circuit design for each origami module consists of two types of Printed Circuit Boards (PCBs): the smart motor drivers soldered to all six N20 motors on the origami actuator and wheel system and a central circuit board mounted within the cross-section of the robot. The central circuit board is responsible for controlling wireless communication and regulates and distributes power for all six smart motor drivers. The smart motor driver contains a microcontroller, a counter, an encoder, and a motor driver onboard. This organization structure allows for the boards to have smaller profiles capable of fitting within the robot's body without sacrificing desired components or ease of communication, which supports modularity and maintainability \cite{KatzWheeler2022}.


% Each separate module contains embedded electronic system, including a 32-bit ARM Cortex processor as the main controller and three sets of motor control chips. Salamanderbot's circuit boards have shrunk in size by nearly half compared with their predecessors, which makes the entire body smaller. Motor sets are placed triangulated on bottom side of the circuit board. By adjusting the motor to pull or release the cable, the module can bend in different directions, thus controlling the movement direction of the module. Specifically, the main controller reads the value of  motor encoders, then calculates and outputs the corresponding PWM for the motors according to the codes. This low-level control mechanism has been illustrated in our prior work \cite{santoso2017design}, either. In addition, a SPI interface is extended on the circuit board, which enables each module to be easily configured into slave mode and receive master board's instruction for high-level tasks.

To enable closed-loop force, velocity, and position control on each degree of freedom, 
%we introduce a smart motor driver control board that can be mounted on the back of small electric motors and used in a broad range of applications beyond the scope of this project. 
the satellite smart motor driver boards are commanded via $I^2C$ by an ESP~32 module mounted on the central circuit board that receives remote commands via WiFi. The microcontroller on each satellite smart driver board control the DC motor through the on board driver, while the encoder and decoder send feedback from the DC motor to the microcontroller for closed-loop position or speed control. 
% As a result, the central circuit board would be responsible for wireless communication, power regulation and distribution, and control of several satellite smart motor driver boards. 
% These smart motor drivers have a micro-controller on board, as well as encoders, current sensors, and other components. This organization structure allows for boards with smaller profiles capable of fitting within the envelope of the robot body, without sacrificing desired components or ease of communication.

The signal flow chart of the entire system is shown in Figure~\ref{signal_flow}.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{Figure/signal_flow_ver2.png}
    \caption{Signal flow of the robot.}      
    \label{signal_flow}
\end{figure}


% The communication / control architecture for operation of CLARA can be broken into two main components, with the first being WiFi communication for control of the robot and the second being I2C
% communication between the main onboard ESP and the smart motor drivers.

% The salamander robot has an origami-inspired continuum body structure with driven wheels on a suspension mechanism, running in closed-loop control to modify the body shape and change length to negotiate pipe networks and adjust force on the tube. The origami body utilizes a Yoshimura crease pattern to achieve continuously deformable cable driven bellows that enable steering by body deformation without traditional rigid mechanisms. To enable closed-loop force, velocity, and position control on each degree of freedom, we introduce a smart motor driver control board that can be mounted on the back of small electric motors and used in a broad range of applications beyond the scope of this project. The motor drivers are commanded via I2C by a custom mainboard that receives remote commands via WiFi and UART from a gamepad or similar user input. The system achieves 4.5” of linear compression, 1.6” of diameter range and 85.8° maximum bending angle. This project provides a foundation for future research into multi-robot inclusion and sensor integration.


==> sections/old-sections/old-demonstration.tex <==
\subsection{Passive Climbing}
The passive suspension design in the propulsion wheel system is supposed to enable the robot to be adaptive to unexpected environment and even utilize the reactive force from the environment to help with propulsion. In order to demonstrate this hypothesis, a modular continuum mobile robot equipped with suspension propulsion wheel system was set in a narrow gap vertical to the ground surface and commanded to drive ``forward" (up, in this case). There was no pre-programmed gait or manual manipulation during the test influencing the origami actuator or the wheel system to ensure that the robot was reacting passively to the environment.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{Figure/go_vertical.png}
    \caption{The modular continuum mobile robot moving vertically along a narrow gap for a body length in 16~s with time stamp.}      
    \label{go_vertical}
\end{figure}


As shown in Figure~\ref{go_vertical}, the passive suspension system and under-actuated origami module passively adapt to the narrow gap while applying normal stress to the gap surfaces, which result in the traction needed for the robot to move vertically upward a body length distance in 16~s. This test demonstrated that the mobile continuum robot is able to passively adapt to an unknown environment with the flexibility of the suspension and origami actuator.

\subsection{Pipe Climbing with Active Suspension}

To investigate the robot's applicability in pipe inspection, the robot was tested in a straight PVC pipe. The robot was first tested with the PVC pipe laid horizontally, and it succeeded upon the first try. The robot was then tested on its ability to traverse this pipe in a vertical configuration as shown in Figure~\ref{go_tube}. This test was originally performed with uncoated TPU wheels, which experienced too much slippage to climb vertically. Once these wheels were replaced with silicone-coated TPU wheels, this test was successful. The robot performed better when the driven wheels followed the passive wheels in a vertical configuration (that is, the driven wheels pushed from the bottom).

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{Figure/go_tube.png}
    \caption{The modular continuum mobile robot moving inside a vertical PVC tube with a 45~degree short-radius bend in 6~s with time stamp.}
    \label{go_tube}
\end{figure}

To test the bending capabilities of the robot within a pipe, a 45~degree short-radius bend was attached to the straight pipe. The robot was first tested with the active-suspension side leading through the bend, which was successful but required many diameter adjustments by the lead screw mechanism to accommodate the changes in diameter at the connection site of the two pipe sections. The robot was then tested with the passive-suspension side leading through the bend, and it succeeded at the same task more easily than the first test.

==> sections/old-sections/old-math_modeling.tex <==
In this section, the inverse kinematics of the origami module and kinematics modeling of the entire robot is discussed and calculated for robot steering control, motion primitive generating, and path prediction.

The inverse kinematics for the origami actuator is generated for predicting the shape of the continuum body during steering angle control. The state of a single module is described with the following three parameters:
\begin{itemize}
    \item $s$: length of the module central or neutral axis;
    \item$\theta$: angle between top and bottom surfaces of the module;
    \item$\phi$: angle of the top surface's normal vector projected onto the bottom surface, relative to the bottom surface.
    %first we make a projection of the top surface's normal on the bottom surface, and $\phi$ is the rotate angle of the projection;
\end{itemize}
As a typical continuum actuator, our inverse kinematics model is based on existing research work (see \cite{jones2006kinematics} for detailed derivation). From this, the relationship between the cable lengths and the three state parameters can be written as:
\begin{equation}
\begin{split}
    & l_1 = 2\sin(\frac{\kappa s}{2})(\frac{1}{\kappa}-d\sin(\phi))\\
    & l_2 = 2\sin(\frac{\kappa s}{2})(\frac{1}{\kappa}+d\sin(\frac{\pi}{3}+\phi))\\
    & l_3 = 2\sin(\frac{\kappa s}{2})(\frac{1}{\kappa}-d\cos(\frac{\pi}{6}+\phi))
\end{split}
    \label{eq:ik}
\end{equation}
In this equation, $l_1$, $l_2$, and $l_3$ represent the lengths of cable 1, cable 2, and cable 3, and $d$ is the distance from the geometric center of the bottom plate to the cable attachment point.

In order to predict the path of the robot under certain inputs using primitive generating, the kinematics model for the modular continuum mobile robot motion is calculated.

The front side of the robot includes an active wheel set with all the electronic modules and the motors for continuum origami module, making up more than half of the total weight.
Considering the fact that the origami structure and back passive wheel set is much lighter than the front side, it is reasonable to assume that the front active wheel set can perform pure rolling while the back passive wheel set can slide laterally when the module deforms.
Other assumptions related to the kinematics model are listed below:
\begin{itemize}
    \item Movement limited to the horizontal plane;
    \item Wheels are point or line contacts with ground and do not deform, which means the radius of wheels stay constant;
    \item Steering axis normal to surface;
    \item Pure rolling for the front wheel set (velocity differential can be created for the two wheels on surface), while the passive back wheel set can slide;
    \item Since the robot moves in an arc with the same curvature of the neutral axis when the module's deformation is constant, the evolving curvature of the robot's trajectory is also the same as the curvature of the neutral axis for short periods;
    \item Angular velocity of motors can be constant.
\end{itemize}
By analyzing the robot motion, we derive the relationship between the curvature variation and robot velocity with the result as follows (notation in these equations are explained in Figure~\ref{kinematics_salamander} and Table~\ref{table:kinematics_parameter}):
$$\Delta \kappa = \frac{4r}{DL}\Delta\alpha$$
$$v=\frac{(\omega_1+\omega_2) r_1}{2}$$

 \begin{figure}
    \centering
    \includegraphics[width=0.4\linewidth]{Figure/kinematics_model.png}
    \caption{Simplified sketch of a single module robot. The pink dumbbell-like shape on two ends represents the two wheel sets of the robot. The bending block in between represent the origami module. Notations on the sketch are explained in Table~\ref{table:kinematics_parameter}.}      
    \label{kinematics_salamander}
\end{figure}

\begin{table}
    \caption{Parameters in the modular continuum mobile robot kinematics modeling.} % title of Table
	\centering % used for centering table
	\begin{tabular}{l l} % centered columns (4 columns)
		\hline\hline %inserts double horizontal lines
		 Parameters & Explanation\\ [1.0ex]
		\hline % inserts single horizontal line
     $L_1, L_2$& length of the cable on the left and right\\[1.0ex]
     $s$& length of the neutral axis\\[1.0ex]
     $L$& original length of $L_1, L_2, s$\\[1.0ex]
     $\theta$& angle between top and bottom layer\\[1.0ex]
     $D$& distance between two wheels\\[1.0ex]
     $\kappa$& curvature of neutral axis\\[1.0ex]
     $\Delta \kappa$& variation of neutral axis curvature\\[1.0ex]
     $r$& radius of the spool on the motor\\[1.0ex]
     $\alpha$& absolute value of rotation angle of the two motors on\\
     & origami module\\[1.0ex]
     $\Delta \alpha$& absolute value of rotational velocity of the two motors\\ & on origami module\\[1.0ex]
     $\omega_1$& rotation velocity of the bottom left motors on wheel set\\[1.0ex]
     $\omega_2$& rotation velocity of the bottom right motors on wheel set\\[1.0ex]
     $v$ & linear velocity of the single module salamander robot\\[1.0ex]
    
    \hline %inserts single line
	\end{tabular}
	\label{table:kinematics_parameter} % is used to refer this
\end{table}

According to this result, the curvature evolves linearly with the motors' rotation angles on the origami module. Since motors' rotation velocities are constant, curvature changes linearly with time, meaning that curvature bends with constant speed. In addition, the last equation shows that the linear velocity of the single module has a linear relationship with the rotational velocity of the motors on wheel mechanism.
Since the motor rotational velocity can be constant in a certain period, the variation of curvature $\Delta \kappa$, which is same as the variation robot trajectory curvature according to the assumption, is linear with the robot's velocity.

A curve whose curvature changes linearly with its curve length is called an Euler spiral. Thus, the motion primitive of the single module robot is a partial Euler spiral when the origami module is deforming. When the curvature stays constant, however, the motion primitive will be an arc with the same curvature as that of the neutral axis.

==> sections/old-sections/old-mechdesign.tex <==
In general, each module of the modular continuum mobile robot consists of a cable-driven origami actuator, a propulsion wheel mechanism, a power package, a remote communication module to receive and send messages individually, and other sensors for certain requirements.
In this section, we mainly introduce the design of origami actuator and the propulsion mechanism with two kinds of suspension.
\subsubsection{Origami Actuator}
The continuum mobile robot consists of one or more 3-DoF flexible origami modules with high torsional resistance (up to 7.311 Nm/rad), based on the origami continuum bending modules presented in our previous work \cite{santoso2017design,luo_orisnake_2018}. Each module behaves as an independent joint, and when one end is fixed, the other side of the module has an approximately hemispherical workspace. The flexible mechanism of these modules makes use of the Yoshimura pattern: a bellows-like origami crease pattern, as shown in Figure~\ref{origami_module}. To establish such a mechanism, three pieces of 7-mil (178-$\mu$m) thick folded plastic (PET) are assembled through tab and slot patterns, following our origami fabrication process outlined in \cite{santoso2017design,onal_origami-inspired_2012}. A sheet of 1/8” thick laser-cut acrylic is attached to either end of the origami body. The rear plate is then attached directly to the rear wheel array discussed in Section \ref{Subsec:wheelsystem}, while the front plate is connected to a 3D-printed case housing three N20 gear DC motors (gear ratio 1:150) and the module control circuit board as shown in Figure~\ref{origami_module}. This case, which separates the motors and circuit board, was added as an improvement to the design presented in our previous work \cite{sun_salamanderbot_2020} to simplify the assembly process and prevent the motors from possible damage on the circuit board. 

\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{Figure/origami_module.png}
    \caption{(left) A piece of Yoshimura origami folding pattern. (right) A cable driven origami module.}      
    \label{origami_module}
\end{figure}

The DC motors control the length of a nylon fishing line that runs from a micro brass spool on the motor's output shaft to the rear acrylic plate.
The origami module can be controlled to shrink and stretch from 57~mm to 148~mm, or bend to the maximum angle of 106~degree.
The total weight of the origami actuator is around 230~g, integrated with actuation, sensing, and control circuits onboard.
% To actuate the module, each motor controls the length of a nylon fishing line that runs from a 3mm-to-3mm brass connector on the motor's output shaft to the rear acrylic plate. The cables are threaded through a series of holes in the origami body, ensuring that the cable always remains perpendicular to the control board and motors and maximizing the bending moment for the module. When all of the cables are the same length, the origami body is straight and can have a maximum length of 148 mm. If all three motors retract their cables, the entire module will contract axially. However, when a motor retracts its cable while the other two motors remain stationary, the differences in cable length will cause the origami module to bend towards the shorter cable. The motors and cables are mounted in a triangular pattern, giving each module a full 3 degrees of freedom (DoF) in the form of bending curvature, bending direction, and segment length, as illustrated in Fig. \verb|---| (UPDATE FIG REF). 

% More details of the kinematics of the module can be found in our prior work \cite{santoso2017design}, which lays out the derivation of the forward and inverse kinematic models of our cable driven continuum origami actuator assuming the shape of the bent actuator to be a circular arc in 3-D space as well as presents the physical properties of the module, such as the axial and torsional stiffness. For reference, the relevant mechanical properties of the original module found in \cite{santoso2017design} are listed here: the total weight is 110 g, integrated with actuation, sensing, and control systems. The origami structure has a 7.311 Nm/rad (0.128 Nm/degree) torsional stiffness while being capable of bending in two directions and changing arc-length down to a fully collapsed state. The module is capable of passively supporting a 1-kg mass at its tip, equivalent to 4 additional serially connected modules, while only bending approximately 6 degrees.


\subsubsection{Passive Suspension Wheel System}
\label{Subsec:wheelsystem}

% Since the development of our previous Salamanderbot prototypes presented in \cite{sun_salamanderbot_2020}, which each utilized a single motor with one of two transmission system designs to actuate the wheels (the first using gears and the latter using belts), several improvements have been made to the propulsion system. 

Compared to the previous prototypes presented in \cite{sun_salamanderbot_2020}, which each utilized a single motor with either a gear-transmission system or belt-transmission system to actuate the wheels, several improvements have been made to the propulsion system. In order to obtain greater stability and adaptability in response to different surroundings, a wheel array with a wider, axially-symmetric base equipped with three motors and suspension capabilities was developed (see Figure~\ref{passive_suspension}). Each array consists of three 3D-printed wheel holders each connected to a corner of a 3D-printed triangular plate via a 3mm shaft. The wheel holder's rotation about the shaft is limited by a rectangular Ninjaflex ``tendon" that is fixed underneath the shaft between the wheel holder and the main plate. The softness of the tendon provides a spring-like force against the wheel holder, providing passive suspension for the wheels. The wheels themselves are attached to the holders using 3mm D shafts, each with a miter gear between the wheels.  

\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{Figure/passive_suspension.png}
    \caption{(left) Assembled passive suspension wheel system. (top-right) Details of the connection between wheel holder and main plate. (bottom-right) Suspension under external force.}      
    \label{passive_suspension}
\end{figure}

To provide front-wheel drive, a motor is attached to each of the wheel holders on the front wheel array using plastic motor brackets. Each motor's output shaft features a miter gear that drives the corresponding wheel-shaft gear. The rear wheel array is not equipped with motors, and thus follows the front array passively. 


\subsubsection{Active Suspension Wheel System}
% this subsection is about the tube traversing mechanism designed by MQP team CLARA (Tim)
Figure~\ref{active_suspension} shows another wheel system design with active suspension. 
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{Figure/active_suspension.png}
    \caption{Active suspension wheel system (left: fully compressed; right: fully expanded).}      
    \label{active_suspension}
\end{figure}
In this mechanism, a slider-crank mechanism was added to adjust the effective diameter of its wheel array actively.  While the mechanism is more complex to manufacture and control than the passive suspension system, it enables it to more easily traverse environments of varying cross-sectional diameter, like pipe networks or collapsed structures. The active suspension features a redesigned triangular base plate with mounting points at each corner and a 0.25~inch bore bearing fixed in the center. A motor, secured to the base plate and housed inside of the hollow origami bellows, turns a 0.25~inch lead screw coupled to its shaft.  As the lead screw rotates, a second plate with an embedded heat-set threaded insert translates along the lead screw. The second plate forces the modified wheel holders to rotate about their hinges (which are attached to the base plate). Thus, the lead screw can be actuated to adjust the position of the crank arm and attached wheel holders, allowing the robot to set the effective diameter of its wheel array from 9.14~cm to 13.3~cm.

Each wheel holder features an affixed motor driving 32~mm wheels. The wheels were printed in a flexible 3D printable material (Ninjaflex) for better compliance and surrounded by DragonSkin 10 silicone tires for increased traction.    




==> sections/old-sections/old-motion_planning.tex <==
In this section, we introduce a motion planning algorithm for the mobile continuum robot. The algorithm should account for obstacles, smoothness, beginning orientation, ending orientation, and maximum curvature.
% Considering the fact that our proposed working environment is narrow. And the path optimizer afterward can change the path a lot. We would like to have a workable motion plan for our robot.
Two possible motion planners, state lattice Based A-star Algorithm and Covariant Hamiltonian Optimization for Motion Planning (CHOMP), are discussed in this section. Both of the planners are programmed and run in MATLAB.

\subsection{State Lattice A-star Based Motion Planner}
Unlike in the traditional A-star searching algorithm, in state lattice based A-star, every time an unexplored child node is visited, several possible paths are created with our kinematics model as the next future possible motion that the robot is able to perform. The possible paths are named "lattices", and the end nodes of these "lattices" are record as an unexplored child node for further searching. Figure~\ref{lattice_astar}~(top) presents the theory of state lattice based A-star algorithm.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.8\linewidth]{Figure/lattice_astar_sketch.png}
%     \caption{A sketch of lattice based A-star searching algorithm. The curves represent the lattice generated from each node. The green curves represent the searching result.}      
%     \label{lattice_astar_sketch}
% \end{figure}


Figure~\ref{lattice_astar}~(bottom) shows a state lattice based A-star for our robot in simulation. The searching process is set to stop once it is close enough to the goal.
However, it is very difficult to make sure the robot can exactly reach the goal with the right orientation in the searching, because the robot can only follow the state lattice to move.
During the searching, the cost for each movement is the same, while it goes infinite while hitting an obstacle. The heuristic is the Euclidean distance between current search node and the goal.

\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{Figure/lattice_astar_n_result.png}
    \caption{(top) A sketch of state lattice based A-star searching algorithm. The curves represent the state lattice generated from each node. The red curves represent the searching result. (bottom) Two examples of state lattice based A-star search with different obstacle configurations. The left trial searched 49735 nodes in 6.36~s to reach a solution. The right trial searched 883165 nodes in 48.89~s}      
    \label{lattice_astar}
\end{figure}

State lattice based A-star motion planner ensures the feasibility of the trajectory generated for the modular continuum mobile robot. However, the incorporation of the orientation constraint does not work well with this planner, which means the beginning or ending orientation of the trajectory cannot be fixed. This limited the performance during situations where the orientation matters.


\subsection{CHOMP Based Motion Planner}
% In this section, we introduce a motion planning algorithm for Salamanderbot. The algorithm is supposed to create a workable motion plan for our robot considering the obstacle, smoothness, beginning orientation, ending orientation, and maximum curvature.

% Considering the fact that our proposed working environment is narrow. And the path optimizer afterward can change the path a lot. We would like to have a workable motion plan for our robot.

% Two options: Lattice Based A* Algorithm and Covariant Hamiltonian Optimization for Motion Planning (CHOMP). While Lattice Based A* would take too much time for searching since technically there could be unlimited numbers of nodes in workspace for searching. Also A* algorithm can not directly have constraint on starting and ending orientation.

% The algorithm we developed is based on CHOMP algorithm. It is consist of the following modules: Gradient descent with regard to obstacle and smoothness, constraint on orientation and maximum curvature, update rules and re-sampling.
% In this section we introduce a motion planner based on CHOMP, which is short for Covariant Hamiltonian Optimization for Motion Planning (\cite{ratliff2009chomp, zucker2013chomp}).

% It is a motion planning method to generate and optimizing trajectories simultaneously for robotic systems, 
CHOMP, which is short for Covariant Hamiltonian Optimization for Motion Planning (\cite{ratliff2009chomp, zucker2013chomp}), is a motion planning method to generate and optimize trajectories simultaneously for robotic systems.
A covariant gradient update ensures it converges to a smooth and collision-free, locally optimal trajectory quickly. Due to the unique properties of CHOMP, related research developed modified motion planning methods based on CHOMP for different situations with novel properties (\cite{mukadam2016gaussian,byravan2014space,kalakrishnan2011stomp}).


This motion planner consist of following modules: Gradient descent with regards to obstacles in the environment and the smoothness of the trajectory itself, constraint deployment on orientation and maximum curvature, and a rule update and resampling procedure. The pseudo code of this motion planner is shown in Algorithm~\ref{alg:CHOMP}.

\SetKwComment{Comment}{/* }{ */}
\begin{algorithm}
\caption{Motion Planning algorithm based on CHOMP}\label{alg:CHOMP}
% \KwData{$n \geq 0$}
% \KwResult{$y = x^n$}
Input: obstacle, end points/orientation, maximum curvature, maximum iteration;

% $y \gets 1$\;
% $X \gets x$\;
% $N \gets n$\;
% \while{$N \neq 0$ or $iteration \geq iteration-max$}{
\For{k = I}{
  $v_{ori} = f_{constraint}(\xi_{k},v_{start},v_{end})$\Comment*[r]{Constraint for orientation}
  $obs_{virt} = f_{virtualobs}(\xi_{k}, curv_{max})$\Comment*[r]{Virtual obstacle}
  
  $[F_{obs},\bigtriangledown F_{obs}] = f_{obstacle}(\xi_{k},obs,obs_{virt},\epsilon)$\;
  $[F_{smooth},\bigtriangledown F_{smooth}] = f_{smooth}(\xi_{k})$\;
  $U(\xi_{k}) = F_{obs}(\xi_{k}) + \lambda F_{smooth}(\xi_{k})$\;
  $\bigtriangledown U(\xi_{k}) = \bigtriangledown F_{obs}(\xi_{k}) + \lambda \bigtriangledown F_{smooth}(\xi_{k})$\;
  
  \If{$U(\xi_{k} < U_{best})$}{
    $\xi_{best} = \xi_{k}$\;
    $U_{best} = U(\xi_{k})$ \Comment*[r]{Record best result}
  }
  
  $\xi_{k+1} = \xi_{k} - \frac{1}{\eta}A^{-1}\bigtriangledown U(\xi_{k}) + \alpha_{const}A^{-1}v_{ori}$\Comment*[r]{Update}
  
  $U$ \Comment*[r]{Restart}
  
}
\end{algorithm}

\subsubsection{Gradient Descent}
In this algorithm, we discretize the trajectory into a set of $n$ points ($q_0,...,q_n$) and compute dynamical quantities via finite differencing. We focus presently on finite dimensional optimization.

During optimization the cost function of a trajectory contains two parts: an obstacle term $F_{obs}$, which measures the cost of being near obstacles; and a smoothness term $F_{smooth}$ to minimize the overall acceleration, which measures dynamical quantities of the robot such as smoothness and acceleration.
We generally assume that $F_{smooth}$ is independent of the
environment.
% $$F_{obs} = \int_{0}^{1} c(\xi(t))||\frac{d}{dt}\xi(t)|| dt$$

\subsubsection{Constraint}
In this section, we introduce the method of constraint deployment for both the ends' orientation and the maximum curvature considering the curvature limitation of the continuum mobile robot.

The orientation constraint is applied utilizing the smooth projection method from the original CHOMP algorithm (\cite{ratliff2009chomp}). The correction vector set is calculated from the current trajectory to the expected position, and then mapped via the metric tensor $A^{-1}$ and vertical mapping matrix for a smooth update. The orientation constraint is deployed on the points near beginning and ending points.


Considering the situation that the correction vector set could have a reduced influence on the trajectory when the angle between the angle between current orientation and expected orientation is around $(2n+1)\pi$, where $n\in \mathbb{Z}$, the angle between the correction vector and the current orientation is clamped between $-\frac{\pi}{6}$ and $\frac{\pi}{6}$.

The procedure of orientation constraint deployment method is listed below:

\begin{itemize}
    \item Calculate a set of vectors from the affected current points to the estimated point;
    \item If the differential angle is too large, ``clamp" it to a certain range to increase the update effect when the angle between the current and expected orientations is around $(2n+1)\pi, n\in \mathbb{Z}$;
    \item Map the vectors vertical to the path;
    \item Map the set of vectors by multiplying $A^{-1}$, then scale it in the path update.  
\end{itemize}
% \begin{itemize}
%     \item Calculate a set of vector from affected current points to estimated point;
%     \item If the differential angle is too large, "clamp" it to a certain range, in case that the vector is too small after mapping;
%     \item Map the vectors vertical to the path;
%     \item Map the set of vector by multiply $A^{-1}$, then scale it in the path update.  
% \end{itemize}

The curvature constraint is applied by adding a virtual obstacle with the circle's center and radius the same as that of the parts exceeding the maximum curvature along the trajectory. The gradient potential generated by the circular obstacle helps to ``push" the trajectory in the next iterations until the maximum curvature decreases to an acceptable value.
The procedure of curvature constraint deployment method is listed below:

\begin{itemize}
    \item Calculate the curvature of each point on the path;
    \item Find the points with curvatures larger than the maximum value;
    \item Create virtual circular obstacles with the same center and radius for these points;
    \item Add the virtual circular obstacle along with existing obstacles to the obstacle field and gradient calculation in the next iteration.
\end{itemize}

\subsubsection{Update rule and re-sampling}
The rule update includes the gradient descent process and the smooth projection. Both of the terms are scaled down to a proper value for better convergence. The update equation is as follows:
$$\xi_{k+1} = \xi_{k} - \frac{1}{\eta}A^{-1}\bigtriangledown U(\xi_{k}) + \alpha_{const}A^{-1}v_{ori}$$

\subsection{Path Following} %\ys{should we keep this or just shrink into a single sentence?}
% LOS algorithm in each iteration:
Given the feasible path for the continuum mobile robot generated by our motion planner, a tracking algorithm named line of sight (LOS) is applied for path tracking (\cite{fossen2003line}). 
Details of the LOS algorithm's procedure in each iteration are listed as follows:
\begin{itemize}
    \item Find the projection point of the robot on the reference path (closest point);
    \item Move the projection forward along the reference path for a certain distance to get the reference point. (If the robot is close to the next way point, then select the next way point as the reference point);
    \item Create a vector from the current position to the reference point as the LOS vector;
    \item Control the robot to follow the LOS vector.
\end{itemize}


\subsection{Motion Planner Deployed on Robot}
Since the CHOMP-based motion planner provides more advantages to our modular continuum mobile robot in regards to time cost, storage space, and constraints implementation, it is selected as the default option for motion plan deployment.

The entire system is implemented and controlled in MATLAB. A motion capture system is used to capture the position and orientation of the robot as the feedback for the PD robot controller. 
The position of obstacles and target are captured and recorded for motion planner. 
After calculating the reference vector with the LOS tracing algorithm, the control signal is sent to the robot through ESP32 WIFI module.
The bottom figure in Figure~\ref{motion_plan_deploy} shows the modular continuum mobile robot traveling to the target while avoiding the objects, with the beginning orientation angle set to be 90~deg and the ending orientation angle set to be 0~deg. The two figures on the top in Figure~\ref{motion_plan_deploy} show the trajectory generated before moving and the path tracked during the experiment.
\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{Figure/motion_plan_deploy_ver3.png}
    \caption{(Top-Left) Motion planning result. The red curve represent the best trajectory generated in planner after 60 iterations in around 0.7~s. (Top-Right) Path tracking during execution. The blue, red, and green points represent the robot position, projection point, and reference point respectively. The orange arrow represents orientation of the robot. (Bottom) Motion planning and path tracking deployed on the modular continuum mobile robot with time stamp.}      
    \label{motion_plan_deploy}
\end{figure}

==> sections/old-sections/path_generation.tex <==
% In this section, we utilized optimization based motion planning method, like CHOMP, which is short for Covariant Hamiltonian Optimization for Motion Planning (\cite{ratliff2009chomp, zucker2013chomp}), to generate and optimize path simultaneously for robotic systems.
% A covariant gradient update ensures that the path converges to a smooth and collision-free, locally optimal path quickly. 
% The optimization based path planner consists of the following modules: Gradient descent with regards to obstacles in the environment and the smoothness of the trajectory itself, and constraint deployment on orientation. Besides, an active obstacle method is deployed in the algorithm to ensure the quick convergence of the path. The pseudo-code of this motion planner is shown in Algorithm~\ref{alg: CHOMP}.

In this section, we leverage optimization-based motion planning techniques, specifically drawing inspiration from CHOMP (Covariant Hamiltonian Optimization for Motion Planning) \cite{ratliff2009chomp, zucker2013chomp}, to craft a path planning and optimization strategy tailored for our inverse kinematics solver. The primary objective of this step is to generate and concurrently optimize a path that serves as a coarse representation of the continuum manipulator's structural configuration within its operational environment.
Our optimization-based path planner comprises the following modules: the gradient descent mechanism, which accounts for obstacle avoidance and intrinsic path smoothness; constraint enforcement on orientation; and the 'active obstacle' strategy, designed to enhance convergence.





% To further enhance convergence speed and obstacle avoidance, we integrate an 'active obstacle' strategy into the algorithm. This strategy dynamically adapts the path to circumvent obstacles, thereby expediting the convergence process. The active obstacle technique proves crucial in complex, dynamic, and unstructured environments where quick and agile responses are paramount.

% For a comprehensive understanding of the motion planning algorithm's functionality and implementation details, we provide the pseudocode of this motion planner in Algorithm~\ref{alg: CHOMP}. This meticulously designed framework forms the foundation of our path planning methodology, enabling the continuum manipulator to navigate its surroundings with precision and efficiency.

\subsubsection{Optimization Based Path Planner}
The optimization based algorithm employs a gradient descent mechanism that operates in tandem with respect to environmental obstacles and the intrinsic smoothness of the path itself. This dual gradient descent approach ensures that the path rapidly converges to a locally optimal, collision-free, and seamlessly continuous path, essential for a reasonable continuum manipulator configuration.
Here we listed the essential equations used to calculate the cost with regard to intrinsic smoothness ($F_{smooth}$), obstacle avoidance ($F_{obs}$), and overall cost ($U(\xi)$) within the optimization framework.
$$F_{smooth} = \frac{1}{2} \int_{0}^{1} ||\frac{d}{dt}\xi(t)||^2 dt$$

$$F_{obs} = \int_{0}^{1} c(\xi(t))||\frac{d}{dt}\xi(t)|| dt$$

$$U(\xi_{k}) = F_{obs}(\xi_{k}) + \lambda F_{smooth}(\xi_{k})$$

$\lambda$ represent the regularization coefficient as a trade off between minimizing the cost function value and minimize the change in average acceleration of the existing trajectory. $\xi(t)$ represents the path, while $t$ represents the index of the way points on path instead of 'time'. $c(\xi)$ represents the cost with regard to obstacles. Generally, $c$ increase when the path is closer to obstacles. The calculation equation of $c(\xi)$ is listed below.

$$c(\xi(t))=\left\{
\begin{array}{cc}
     -d(\xi(t))+\frac{1}{2}\epsilon,& if~d(\xi(t))<0 \\
     \frac{1}{2\epsilon} (d(\xi(t))-\epsilon)^2,& if~0\leq d(\xi(t)) \leq \epsilon\\
     0, & otherwise
\end{array}
\right.
$$

$d(\xi)$ represents the distance between path $\xi$ and the obstacles. $\epsilon$ represents the maximum distance that the obstacle still have influence on the path during optimization procedure.

% To perform gradient descent, first we approximate the cost function with a first-order Taylor expansion:
% $$U(\xi) \approx U(\xi_k)+\bigtriangledown U(\xi_k)^T(\xi-\xi_k)$$

Moreover, our method incorporates constraint enforcement on orientation, guaranteeing that the continuum manipulator adheres to the desired initial orientation, which will be discussed in a following subsection.

\subsubsection{Active Obstacle}
To expedite convergence, we incorporate the 'active obstacle' method, drawing inspiration from a commonly employed strategy in finite element engineering programs. This method involves gradually increasing the load during simulation until it reaches the required threshold, effectively minimizing step sizes and reducing the likelihood of divergence.

Within our algorithm, we categorize obstacles into two groups, split by the continuum manipulator, temporarily displacing them before returning them to their original positions. The obstacle group are decided by the desired position of the continuum manipulator in the intricate workspace. This 'push-pull' technique gently nudges the path towards the correct alignment with the obstacles. During this process, an artificial potential field generated in relation to the obstacles gradually increases in influence as they move from a distant to a close proximity to the path. This procedure minimizes the step sizes for a better converge, and increases the likelihood that the paths stay in the correct 'valley' in the artificial potential field. 
Optimization continues until the path reaches the desired length, at which point it represents the initial configuration for subsequent updates.




\subsubsection{Updating Rule}
%The updating rule includes the gradient descent process and the smooth projection. Both of the terms are scaled down to a proper value for better convergence. Besides, we also consider the orientation of the continuum manipulator, thus the orientation constraint is applied to utilize the smooth projection method from the original CHOMP algorithm (\cite{ratliff2009chomp}). The correction vector set is calculated from the current trajectory to the expected position, and then mapped via the metric tensor $A^{-1}$ and vertical mapping matrix for a smooth update. The orientation constraint is deployed on the points near the beginning and ending points.

The update rule encompasses two pivotal components: gradient descent for obstacle avoidance and intrinsic smoothness. To enhance convergence, both terms are appropriately scaled.

Furthermore, we integrate orientation considerations into our methodology to ensure that the continuum manipulator maintains the desired initial orientation. This orientation constraint utilizes the smooth projection method, incorporated in the CHOMP algorithm, to confine the path within the designated workspace \cite{ratliff2009chomp}.
The correction vector set is calculated by assessing the deviation between the current path and its expected position. This set of correction vectors is then transformed using the metric tensor $A^{-1}$ and a vertical mapping matrix, which collectively facilitate a seamless update of the path.

% Notably, we apply the orientation constraint selectively, focusing on points in close proximity to the beginning and ending segments of the path. This strategic deployment of the orientation constraint ensures that the manipulator conforms to orientation specifications during crucial phases of its operation.



% \ys{rearrange the stuff below, maybe send to other sections}

% The pseudo code of this motion planner is shown in Algorithm~\ref{alg:CHOMP}.

% \SetKwComment{Comment}{/* }{ */}
% \begin{algorithm}
% \caption{Path Planning algorithm with Active Obstacle}\label{alg:two}
% % \KwData{$n \geq 0$}
% % \KwResult{$y = x^n$}
% Input: obstacle, end points/orientation, maximum curvature, maximum iteration;

% % $y \gets 1$\;
% % $X \gets x$\;
% % $N \gets n$\;
% % \while{$N \neq 0$ or $iteration \geq iteration-max$}{
% \For{k = I}{
%   $v_{ori} = f_{constraint}(\xi_{k},v_{start},v_{end})$\Comment*[r]{Constraint for orientation}
%   $obs_{virt} = f_{virtualobs}(\xi_{k}, curv_{max})$\Comment*[r]{Virtual obstacle}
  
%   $[F_{obs},\bigtriangledown F_{obs}] = f_{obstacle}(\xi_{k},obs,obs_{virt},\epsilon)$\;
%   $[F_{smooth},\bigtriangledown F_{smooth}] = f_{smooth}(\xi_{k})$\;
%   $U(\xi_{k}) = F_{obs}(\xi_{k}) + \lambda F_{smooth}(\xi_{k})$\;
%   $\bigtriangledown U(\xi_{k}) = \bigtriangledown F_{obs}(\xi_{k}) + \lambda \bigtriangledown F_{smooth}(\xi_{k})$\;
  
%   \If{$U(\xi_{k} < U_{best})$}{
%     $\xi_{best} = \xi_{k}$\;
%     $U_{best} = U(\xi_{k})$ \Comment*[r]{Record best result}
%   }
  
%   $\xi_{k+1} = \xi_{k} - \frac{1}{\eta}A^{-1}\bigtriangledown U(\xi_{k}) + \alpha_{const}A^{-1}v_{ori}$\Comment*[r]{Update}
  
%   $U$ \Comment*[r]{Restart}
  
% }\label{alg:CHOMP}
% \end{algorithm}





% In order to make small changes in the average acceleration of the resulting trajectory as possible, an extra term $\frac{\lambda}{2}(\xi-\xi_k)^TA(\xi-\xi_k)$ is added, thus, the optimization problem becomes:
% \begin{equation}
% \begin{aligned}
%     \xi_{k+1} =\mathop{\arg\min}\limits_{\xi}\left \{ U(\xi_k)+\bigtriangledown U(\xi_k)^T(\xi-\xi_k)+ \frac{\lambda}{2}(\xi-\xi_k)^TA(\xi-\xi_k)\right \}
% \end{aligned}
% \end{equation}


% \ys{rearrange the stuff upward, maybe send to other sections}


As a result the gradient descent update rule can be written as follows:
$$\xi_{k+1}=\xi_k-\frac{1}{\lambda} A^{-1}\bigtriangledown U(\xi_k)+ \alpha_{const}A^{-1}v_{ori}$$
$\xi$ keeps updating until the total length reaches the target value (the length of the entire continuum manipulator), or when it reaches the maximum iteration.

The update of our optimization based path plan algorithm is shown in Figure~\ref{path_plan}


\begin{figure}
    \centering
    \includegraphics[width=1.0\linewidth]{Figure/path_plan.png}
    \caption{Path plan algorithm within 28 iterations. The circles represent the obstacles, and the dashed line represents the path connecting two ends. The 'active obstacles' have been in position and stopped to move since the $12^{th}$ iteration.}      
    \label{path_plan}
\end{figure}

==> sections/old-sections/reviews.tex <==
1.Circular spline fitting using an evolution process\cite{song2009circular}
Contributions:
\begin{itemize}
    \item 1.an independent set of shape parameters, which uniquely
describe a circular spline curve;
    \item 2.an evolution process (governed by a differential equation) for circular spline curves in 3d;
    \item 3.demonstrate that circular spline curves for curve fitting has advantage of simple and explicit closest point computation
\end{itemize}

Recently, circular splines have been used for reconstructing pipe surfaces from unorganized measurement data by Bauer
and Polthier [2] A moving least-squares-based technique is used to reconstruct the spine curve of a pipe surface from surface
samples and approximate the spine curve by G1 continuous circular arcs and line segments.\\
Gauss–Newton-type techniques


